Composable Rate-Independent Computation in Continuous Chemical Reaction Networks

Biological regulatory networks depend upon chemical interactions to process information. Engineering such molecular computing systems is a major challenge for synthetic biology and related fields. The chemical reaction network (CRN) model idealizes chemical interactions, allowing rigorous reasoning about the computational power of chemical kinetics. Here we focus on function computation with CRNs, where we think of the initial concentrations of some species as the input and the equilibrium concentration of another species as the output. Specifically, we are concerned with CRNs that are rate-independent (the computation must be correct independent of the reaction rate law) and composable ($f\circ g$ can be computed by concatenating the CRNs computing $f$ and $g$). Rate independence and composability are important engineering desiderata, permitting implementations that violate mass-action kinetics, or even "well-mixedness", and allowing the systematic construction of complex computation via modular design. We show that to construct composable rate-independent CRNs, it is necessary and sufficient to ensure that the output species of a module is not a reactant in any reaction within the module. We then exactly characterize the functions computable by such CRNs as superadditive, positive-continuous, and piecewise rational linear. Thus composability severely limits rate-independent computation unless more sophisticated input/output encodings are used.

==> FROM_OLD_PAPER_prelim.tex <==
% !TEX root = main.tex


\section{Preliminaries}
\label{sec-prelim}

Let $\N$ and $\R$ denote the set of nonnegative integers and the set of real numbers, respectively.
If $x \in \R$, let $\R_{\geq x} = \setr{x'\in\R}{x' \geq x}$, and similarly for $\R_{> x}$.
Given a vector $\vx\in\R^k$, let $\|\vx\| = \|\vx\|_1 = \sum_{i=1}^k \vx(i)$, where $\vx(i)$ denotes the $i$th coordinate of $\vx$.
We abuse notation and consider the sets $\R^k \times \R^l$ and $\R^{k+l}$ to be the same, because it is sometimes convenient to treat an ordered pair of vectors as being concatenated into a single longer vector.
If $\Lambda$ is a finite set (in this paper, of chemical species), we write $\R^\Lambda$ to denote the set of functions $f:\Lambda \to \R$, and similarly for $\Rp^\Lambda$, $\N^\Lambda$, etc.
Equivalently, we view an element $\vc\in A^\Lambda$ as a vector of $|\Lambda|$ elements of $A$, each coordinate ``labeled'' by an element of $\Lambda$.
%Write $\vc \rest \Delta$ to denote the vector $\vd \in A^\Delta$ such that $\vc(S)=\vd(S)$ for all $S \in \Delta$.


\subsection{Chemical reaction networks}
Given $S\in \Lambda$ and $\vc \in \Rp^\Lambda$, we refer to $\vc(S)$ as the \emph{concentration of $S$ in $\vc$}.
For any $\vc\in \Rp^\Lambda$, let $[\vc] = \{S \in \Lambda \ |\ \vc(S) > 0 \}$, the set of species \emph{present} in $\vc$.
%We also equivalently view an element $\vc \in \N^\Lambda$ as a \emph{multiset} of elements of $\Lambda$, where $\vc(X)$ is the multiplicity of element $X \in \Lambda$.
%We therefore write $\vc \subseteq \vc'$ to denote that $\vc(X) \leq \vc'(X)$ for all $X \in \Lambda$.
We write $\vc \leq \vc'$ to denote that $\vc(S) \leq \vc'(S)$ for all $S \in \Lambda$.
Given $\vc,\vc' \in \Rp^\Lambda$, we define the vector component-wise operations of addition $\vc+\vc'$, subtraction $\vc-\vc'$, and scalar multiplication $x \vc$ for $x \in \R$.
If $\Delta \subset \Lambda$, we view a vector $\vc \in \Rp^\Delta$ equivalently as a vector $\vc \in \Rp^\Lambda$ by assuming $\vc(S)=0$ for all $S \in \Lambda \setminus \Delta.$
For $\Delta \subset \Lambda$, we write $\vc  \upharpoonright \Delta$ to denote $\vc$ \emph{restricted to} $\Delta$; in particular, $\vc  \upharpoonright \Delta = \vec{0} \iff (\forall S\in\Delta)\ \vc(S)=0.$


Given a finite set of chemical species $\Lambda$, a \emph{reaction} over $\Lambda$ is a pair $\alpha = \langle \bfr,\bfp \rangle \in \N^\Lambda \times \N^\Lambda$, specifying the stoichiometry of the reactants and products, respectively.\footnote{It is customary to define, for each reaction, a \emph{rate constant} $k \in \R_{>0}$ specifying a constant multiplier on the mass-action rate (i.e., the product of the reactant concentrations), but as we are studying CRNs whose output is independent of the reaction rates, we leave the rate constants out of the definition.} %, and the \emph{rate constant} $k$.
In this paper, we assume that $\bfr \neq \vec{0}$, i.e., we have no reactions of the form $\emptyset \to \ldots$.\footnote{We allow high order reactions; i.e., those that consume more than two reactants.
It is not difficult to show that such a reaction $S_1 + S_2 + \ldots + S_n \to P_1 + \ldots + P_m$ can be replaced by bimolecular reactions $S_1 + S_2 \revrxn S_{12}, S_{12} + S_3 \revrxn S_{123}, S_{123} + S_4 \revrxn S_{1234}, \ldots, S_n + S_{12 \ldots n-1} \to P_1 + \ldots + P_m$ without affecting the correctness of the CRN.}
%If not specified, assume that $k=1$, so that the reaction $\alpha=\langle \bfr,\bfp,1 \rangle$ is also represented by the pair $\pair{\bfr}{\bfp}.$
For instance, given $\Lambda=\{A,B,C\}$, the reaction $A+2B \to A+3C$ is the pair $\pair{(1,2,0)}{(1,0,3)}.$
Note that we represent reversible reactions such as $A \revrxn B$ as two irreversible reactions $A \to B$ and $B \to A$.
A \emph{(finite) chemical reaction network (CRN)} is a pair $\calC=(\Lambda,R)$, where $\Lambda$ is a finite set of chemical \emph{species},
%$\Sigma \subseteq \Lambda$ be a finite \emph{input alphabet} (a.k.a., \emph{set of input species}), $\phi:\Lambda\to\{0,1\}$ is the \emph{output function},
and $R$ is a finite set of reactions over $\Lambda$.
A \emph{state} of a CRN $\calC=(\Lambda,R)$ is a vector $\vc \in \Rp^\Lambda$.
Given a state $\vc$ and reaction $\alpha=\pair{\bfr}{\bfp}$, we say that $\alpha$ is \emph{applicable} in $\vc$ if $[\bfr] \subseteq [\vc]$ (i.e., $\vc$ contains positive concentration of all of the reactants).




















\subsection{Reachability}
\label{subsec-reachability}


In the previous section we defined the syntax of CRNs.
We wish to define a semantic interpretation of them suitable for defining how they compute functions.
In particular, we want to consider CRNs guaranteed to correctly compute a function of their inputs, regardless of the rate at which reactions proceed, calling this \emph{stable computation}, defined in Section~\ref{subsec-stable-crns}.
This definition rests on another, which we must take care in defining, namely what it means for one state to be \emph{reachable} from another, which is the focus of this section.
Intuitively, $\vd$ is reachable from $\vc$ if applying some amount of reactions to $\vc$ results in $\vd$, such that no reaction is ever applied when any of its reactants are concentration 0.
Formalizing this concept is a bit tricky and constitutes one of the contributions of this paper.
%We give two formal definitions, one that appears to formally capture what we just described, and another that seems more restrictive but is easier to work with, and we prove that the latter can be used to give an equivalent definition of the former.
Intuitively, we'll think of reachability via straight line segments.
This may appear overly limiting; after all mass-action and other rate laws trace out smooth curves.
However we show a number of properties of our definition that support its reasonableness.
%Indeed, we will show that our definition is more general than mass-action.
%Importantly, our positive results in the following sections (constructions computing functions) work under mass-action kinetics, and thus do not rely on the generalized notion of reachability.


Throughout this section, fix a CRN $\calC = (\Lambda,R)$.
All states $\vc$, etc., are assumed to be states of $\calC$.
Let $m=|R|$ be the number of reactions in CRN $\calC$, and let $n = |\Lambda|$ be the number of species in $\calC$.
We define the $n \times m$ \emph{reaction stoichiometry matrix} $\vM$ such that
$\vM(i,j)$ is the net amount of the $i$'th species that is produced by the $j$'th reaction (negative if the species is consumed).\footnote{Note that $\vM$ does not fully specify $\calC$, since catalysts are not modeled: reactions $Z + X \to Z + Y$ and $X \to Y$ both correspond to the column vector $(-1,1,0)^\top$.}
\opt{normal,itcs}{For example, if we have the reactions $X \to Y$ and $X + A \to 2X + 3Y$, and if the three rows correspond to $X$, $A$, and $Y$, in that order, then
  $$
    \vM =
    \left(
      \begin{array}{cc}
        -1 & 1 \\
        0 & -1 \\
        1 & 3 \\
      \end{array}
    \right)
  $$
}
%TODO: formally define M in terms of reactions (\vr,\vp)


\begin{definition}\label{defn-reachable-line}
State $\vd$ is \emph{straight-line reachable (aka $1$-segment reachable)} from $\vc$, written $\vc \slto \vd$, if $(\exists \vu \in \Rp^m)\ \vc + \vM \vu = \vd$
and $\vu(j) > 0$ only if reaction $j$ is applicable at $\vc$.
In this case write $\vc \slto_\vu \vd$.
\end{definition}

Intuitively, by a single segment we mean running the reactions applicable at $\vc$ at a constant (possibly 0) rate to get from $\vc$ to $\vd$.
In the definition, $\vu(j)$ represents the flux of reaction $j$.


\begin{definition}\label{defn-reachable-lines}
State $\vd$ is \emph{$l$-segment reachable}, written $\vc \segto^l \vd$ from $\vc$ if $(\exists \vb_1, \dots, \vb_{l+1})\ \vc  = \vb_1 \slto \vb_2 \slto \vb_3 \slto \dots  \slto \vb_{l+1} = \vd.$
\end{definition}


\begin{definition}\label{defn-reachable-segment}
State $\vd$ is \emph{segment-reachable} from $\vc$, written $\vc \segto \vd$, if $(\exists l\in\N)\ \vc \segto^l \vd$.
\end{definition}


Suppose the reactions are $X \to C$ and $C + Y \to C + Z$, and we are in state $\{0 C, 1 X, 1 Y, 0 Z\}$.
With straight-line segments, any state with a positive amount of $Z$ must be reached in at least two segments: first to produce $C$, which allows the second reaction to occur, and then any combination of the first and second reactions.
For example,
\opt{normal,submission,final}{$\{0 C, 1 X, 1 Y, 0 Z\}  \slto  \{0.1 C, 0.9 X, 1 Y, 0 Z\} \slto  \{1 C, 0 X, 0 Y, 1 Z\}$}
\opt{itcs}{$\{0 C$, $1 X$, $1 Y$, $0 Z\}$  $\slto$  $\{0.1 C$, $0.9 X$, $1 Y$, $0 Z\}$ $\slto$  $\{1 C$, $0 X$, $0 Y$, $1 Z\}$.}
This is a simple example showing that more states are reachable with $\segto$ than $\slto$.
Often Definition~\ref{defn-reachable-segment} is used implicitly, when we make statements such as, ``Run reaction 1 until its first reactant is 0, then run reaction 2'', which implicitly defines two straight lines in concentration space.

Given a curve, we can think about approximating it to an arbitrary accuracy using straight-line segments.
But it may seem that we can never achieve the ``full diversity'' of states reachable with curves if we use only a finite number of line segments.
However, the following lemma shows that increasing the number of straight-line segments beyond a certain point does not make any additional states reachable.
Thus using a few line segments captures all the states reachable in the limit of infinitely many line segments.
\opt{submission}{A proof of the following lemma is given in the appendix.}
\opt{final}{A proof of the following lemma is given in the full version.}



\newcommand{\lemReachableSegmentBound}
{If $\vc \segto \vd$, then $\vc \segto^{m+1} \vd$, where $m=|R|$ is the number of reactions.}

\begin{lemma}\label{lem-reachable-segment-bound}
  \lemReachableSegmentBound
\end{lemma}

\newcommand{\proofLemReachableSegmentBound}{
\begin{proof}
    The intuitive idea of the proof is as follows.
    If $\vc \segto \vd$, then the path could use a huge number of segments, much greater than $m+1$.
    We don't care precisely what these segments are, only that they give us an \emph{ordering $\prec$ on species that need to become positive to reach $\vd$}, such that, calling the species $S_1 \prec S_2 \prec \ldots \prec S_p$, for each $i$, there is a reaction to produce $S_i$ that has only reactants in $[\vc] \cup \{S_1,\ldots,S_{i-1}\}$.
    Therefore we can produce a small amount of each species $S_1,\ldots,S_n$, starting only from species in $[\vc]$, by running these reactions in order, and running each reaction a smaller amount than the previous to ensure that nothing positive goes to 0.
    Once all these species are produced, a single straight line can take the CRN to state $\vd$.
    The trick is that we should not produce \emph{every} producible species, but only those needed to run the reactions corresponding to the final straight line.
    Otherwise, for example, we could create a species $X \not\in [\vc] \cup [\vd]$, and if no reaction consumes $X$, $\vd$ would become unreachable.

    If $\vd$ is reachable from $\vc$ via fewer than $m+1$ straight line segments, then this can be re-expressed with precisely $m+1$ line segments by using length-0 line segments.
    It remains to show that at most $m+1$ straight line segments are necessary.

    Suppose that $\vc \segto \vd$ via $l > m+1$ straight line segments $\vc=\vb_0 \slto \vb_1 \slto \ldots \slto \vb_l = \vd$.
    Let the reactions $R$ be ordered as $\alpha_0, \alpha_1,\ldots.$
    For each $\vb_i$, there exists $\vu_i$ such that $\vb_{i} + \vM \vu_i = \vb_{i+1}$.
    Let $F_j = \sum_{i=0}^{l-1} \vu_i(j)$ be the total flux through reaction $\alpha_j$ to get from $\vc$ to $\vd$ along the $l$ straight line segments defined by the $\vb_i$'s.
    Let $P = \setr{j}{F_j > 0}$ be the indices of reactions that occurred with strictly positive flux.
    If $\alpha_j=(\vr_j,\vp_j)$, let $\vv_j = \vp_j-\vr_j$ be the vector representing the net change in concentrations if reaction $\alpha_j$ experiences unit flux.
    Then $\vd = \vc + \sum_{j \in P} F_j \vv_j$.
    We use this fact to show that $\vc \segto^{m+1} \vd$.

    Let $R(P) = \setl{\alpha_j\in R}{j \in P}$ be the reactions with indices in $P$.
    We first argue that there is an ordering $\prec$ of reactions in $R(P)$, such that for any reaction $\alpha=(\vr,\vp)$, $[\vr] \subseteq [\vc] \cup \bigcup_{\alpha'=(\vr',\vp') \prec \alpha} [\vp']$.
    In other words, if all products of reactions preceding $\alpha$ have positive concentration, as well as all species present in $\vc$, this guarantees $\alpha$ is applicable.
    This in turn allows the reactions to proceed in the given order, so long as we are careful that no positive concentration species is allowed to be consumed back to 0.
    At the end, all products of all reactions in $R(P)$ are positive.
    To see that this ordering exists, it suffices to observe that the straight line segments given by the hypothesis $\vc \segto \vd$ give a \emph{partial} order that respects the constraints, since any reactions with positive flux in the $k$'th straight line segment, which were not positive flux in any previous straight line segments, must consume only species that were either positive in $\vc$, or that were produced by a reaction with positive flux in the $l$'th straight line segment, where $l < k$.
    Given all reactions having positive flux for the first time in the $k$'th straight line segment, they can be ordered arbitrarily relative to each other while obeying the constraint $\prec$.
    For the sake of brevity, assume without loss of generality that $P = \{0,1,\ldots,|P|-1\}$, and that $\alpha_0 \prec \alpha_1 \prec \ldots \prec \alpha_{|P|-1}$.


    Let $K = \max_{S \in \Lambda} \max_{\alpha=(\vr,\vp)\in R(P)} \vr(S)$ be the maximum stoichiometry coefficient of any possible reactant.
    In the worst case, running a reaction by $\delta$ flux will decrease the concentration of any species by at most $\delta K$.
    Let
    \opt{normal,submission}{$\epsilon = \min \left\{ \min_{S \in [\vc]} \vc(S), \min_{j \in P} F_j \right\}.$}
    \opt{itcs,final}{\[\epsilon = \min \left\{ \min_{S \in [\vc]} \vc(S), \min_{j \in P} F_j \right\}.\]}
    The significance of $\epsilon$ is that if we allow all reactions in $R(P)$ to go forward from $\vc$ by strictly less than $\epsilon$ of flux, this will be less than the total flux experienced by each reaction, and also each species present in $\vc$ will remain in positive concentration.
    Formally, define the following basis vectors (representing individual reaction vectors) $\vw_j\in\Rp^m$ for $0 \leq j < |P|$.
    Let $\vw_j(j) = \frac{\epsilon}{(2K)^{j+1}}$ and $\vw_i(j) = 0$ if $i \neq j$.
    Then $\vM \vw_j$ is the $j$'th line segment to define.
    Let $\va=\vc+\sum_{j=0}^{|P|-1} \vM \vw_j$ be the point reached after following these line segments.
    For each $j$, let $\va_{j} = \vc + \sum_{i=0}^{j-1} \vM \vw_{i}$ be the state reached after following the first $j$ straight line segments, letting $\va_0=\vc$.

    We prove by induction on $j$ that each $\vM \vw_j$ satisfies Definition~\ref{defn-reachable-line} by showing that for all $j$, $S \in [\va_j] \implies \va_j(S) \geq \frac{\epsilon}{(2K)^{j+1}}$.
    I.e., all species are nonnegative at the start and end of the line (hence along the entire line), and the reactions experiencing positive flux along the line are applicable at the starting state.

    We first establish the base case, where $\vw_0(0) = \frac{\epsilon}{2K}$.
    By the definition of $\prec$, which ensures that for $\alpha_0=(\vr_0,\vp_0)$, $[\vr_0] \subseteq [\vc]$, $\alpha_0$ is applicable at $\vc$.
    Note that $\epsilon \leq \vc(S)$ for all $S \in [\vc]$, i.e., running $\alpha_0$ with flux $\frac{\epsilon}{2K}$ can cut the concentration of any species $S \in [\vc]$ at most in half, so that in state $\va_1 = \vc + \vM \vw_0$, $\va_1(S) \geq \frac{\epsilon}{2} \geq \frac{\epsilon}{2K}$, satisfying the base case for species in $[\vc]$.
    Because $\alpha_0$ experiences $\frac{\epsilon}{2K}$ of flux, each species produced $S \in [\vp_0] \setminus [\vc]$ initially absent in $\vc$ but produced in $\va_1$ has increased in concentration by at least $\frac{\epsilon}{2K}$.
    Therefore all species in $[\va_1] \setminus [\vc]$ have concentration at least $\frac{\epsilon}{2K}$, satisfying the base case for these species.

    For the inductive case, inductively assume each species $S \in [\va_j]$ satisfies $\va_j(S) \geq \frac{\epsilon}{(2K)^{j+1}}$.
    Then by the definition of $\alpha_j$ and $\prec$, $\alpha_j$ is applicable in $\va_j$.
    Similarly to the base case, by running $\alpha_j$ by flux $\frac{\epsilon}{(2K)^{j+2}}$, the most any such species is consumed is $\frac{\epsilon}{(2K)^{j+2}}$, and since all such species $S$ started with concentration $\va_j(S) \geq \frac{\epsilon}{(2K)^{j+1}}$, their concentrations are at most cut in half, i.e. $\va_{j+1}(S) \geq \frac{\epsilon}{(2K)^{j+2}}$.
    Therefore the inductive hypothesis for case $j+1$ is satisfied for species in $\va_j$.
    To show that the inductive hypothsis is satisfied for the rest of the species (i.e., those in $[\va_{j+1}] \setminus [\va_j]$), observe that all products $S \in [\va_{j+1}] \setminus [\va_j]$ have increased in concentration by at least $\frac{\epsilon}{(2K)^{j+2}}$.

    The final line segment is a straight line from $\va$ to $\vd$.
    By our choice of $P$, all reactions in $R(P)$ are applicable at $\va$.
    By our choice of $\vw_j$'s, the total flux experienced by reaction $\alpha_j$ to get from $\vc$ to $\va$ is strictly less than $F_j$, the total flux $\alpha_j$ experienced in the original straight line segments defining $\vc \segto \vd$.
    Therefore the final straight line from $\va$ can be defined by the vector $\vw(j)=F_j-\vw_j(j)$, so that $\va + \vM \vw = \vd$.
    This shows that $\vc \segto^{m+1} \vd$.
\end{proof}
}
\opt{normal,itcs}{\proofLemReachableSegmentBound}





%\vspace{10pt}

\subsection{Relation to mass-action}
For understanding the results of this paper, it is not necessary to be familiar with mass-action kinetics.
However, as mass-action is the most commonly used model of chemical kinetics, we want to be satisfied that our notion of reachability at least considers states that can be reached by mass-action trajectories.
Indeed, Lemma~\ref{lem:mass-action-reachable} shows that our notion of reachability is more general than mass-action.


While a thorough discussion of mass-action kinetics is beyond the scope of this paper,
we remind the reader that a CRN with rate constants assigned to each reaction defines a mass-action ODE system with a variable for each species.
Each reaction contributes a term to the ODEs for all the species participating in it (except catalysts that are unchanged in the reaction).
The term from reaction $\alpha$ appearing in the ODE for $x$ is the product of:
the rate constant,
the reactant concentrations,
and the net stoichiometry of $x$ in $\alpha$.
For example, the CRN
\begin{align*}
X + X &\to C \\
C + X &\to C + Y
\end{align*}
corresponds to ODEs:
\begin{align*}
\dot{x} &= -2 k_1 x^2 - k_2 c x \\
\dot{c} &= k_1 x^2 \\
\dot{y} &=  k_2 c x
\end{align*}
where $k_1, k_2$ are the rate constants of the two reactions.
We restrict our attention to CRNs whose mass-action trajectories are well-defined at all times $t \geq 0$, and where concentrations remain finite for all finite $t$.\footnote{Although mass-action systems are free of many pathologies of more general dynamical systems, there are mass-action CRNs that reach infinite concentration in finite time: e.g.~$2X \to 3X$}



\begin{definition}
A state $\vd$ is \emph{mass-action reachable} from $\vc$ if there are non-zero rate constants such that the corresponding mass-action trajectory starting in $\vc$ passes through $\vd$, or approaches $\vd$ as $t \rightarrow \infty$.
\end{definition}


%Of course, it is insufficient to justify our reachability relation solely on the basis that it is a superset of the mass-action reachability relation; the relation that states every state is reachable from every other state has this property as well but is unconnected to the reactions of the CRN.
%Ultimately, we must appeal to intuition to justify that our definition does not reach too far.
%Our intuition says that the following properties (achieved by our definition but conceivably acheived by alternatives) are required of any reasonable notion of reachability: 1) a reaction cannot execute in any state in which some reactant is 0,\footnote{In particular, we want that ``siphons'', defined below, should behave the same; i.e., that Lemmas~\ref{lem-mass-action-forward-invariant-siphon} and~\ref{lem-seg-reachable-forward-invariant-siphon} should apply to any reasonable notion of reachability.} 2) concentrations must be nonnegative in all reachable states, 3) the relation should be reflexive, transitive, and ``respect addition'' (if $\vx\to\vy$, then for all $\vc$, $\vx+\vc\to\vy+\vc$, since the presence of additional chemicals should not \emph{prevent} reactions from being possible).
%Our definition was the most general one we could conceive that satisfied these properties.


In order to prove Lemma~\ref{lem:mass-action-reachable} we need to introduce the notion of a \emph{siphon} from the Petri net literature.
This notion will be used, as well, to prove negative results in later sections.
Let $\calC=(\Lambda,R)$ be a CRN.
A \emph{siphon} is a set of species $\Omega \subseteq \Lambda$ such that, for all reactions $\alpha=(\vr,\vp) \in R$, $[\vp] \cap \Omega \neq \emptyset \implies [\vr] \cap \Omega \neq \emptyset$, i.e., every reaction that produces an element of $\Omega$ requires a positive concentration of an element of $\Omega$ to be applicable.
The following lemma, due to Angeli, De Leenheer, and Sontag~\cite{angeli2007petri}, shows that this is equivalent to the notion that ``the absence of $\Omega$ is forward-invariant'' under mass-action: if all species in $\Omega$ are absent, then they can never again be produced (under mass-action).\footnote{It may appear obvious that if the rates of all reactions producing a particular species are zero, the species cannot be produced.
However, this is a rather deep fact about mass-action ODEs.
Consider the CRN $2X \to 3X$. The corresponding mass-action ODE is $\dot{x} = x^{2}$, and has the property that if you start with $x(0) = 0$, it cannot become positive.
However, the very similar non-mass-action ODE
$\dot{x} = x^{1/2}$
has a perfectly valid solution $x(t) = t^2/4$ which starts at $0$ but becomes positive,
despite the fact that at $t=0$, $\dot{x} = 0$.
}
%\todo{Explain why this is a deep fact and non-obvious}




\begin{lem}[\cite{angeli2007petri}]\label{lem-mass-action-forward-invariant-siphon}
  Let $\Omega \subseteq \Lambda$ be a set of species.
  Then $\Omega$ is a siphon if and only if, for any state $\vc$ such that $\Omega \cap [\vc] = \emptyset$ and any state $\vd$ that is mass-action reachable from $\vc$, $\Omega \cap [\vd] = \emptyset$.
\end{lem}

We show that the same holds true for segment-reachability.
\opt{submission}{The following two lemmas are proven in the appendix.}
\opt{final}{The following two lemmas are proven in the full version.}

\newcommand{\lemSegReachableForwardInvariantSiphon}{
  Let $\Omega \subseteq \Lambda$ be a set of species.
  Then $\Omega$ is a siphon if and only if, for any state $\vc$ such that $\Omega \cap [\vc] = \emptyset$ and any state $\vd$ such that $\vc \segto \vd$, $\Omega \cap [\vd] = \emptyset$.
}
\begin{lem}\label{lem-seg-reachable-forward-invariant-siphon}
  \lemSegReachableForwardInvariantSiphon
\end{lem}

\newcommand{\proofLemSegReachableForwardInvariantSiphon}{
\begin{proof}
  Suppose $\Omega$ is a siphon, let $\vc$ be a state such that $[\vc] \cap \Omega = \emptyset$, and let $\vd$ be such that $\vc \segto \vd$.
  Every straight line with end points $\vb_i$ and $\vb_{i+1}$ in the path from $\vc$ to $\vd$ is expressible as a sum of reaction vectors for reactions applicable in $\vb_i$.
  Assuming inductively that $[\vb_i] \cap \Omega = \emptyset$, the definition of siphon gives that $[\vb_{i+1}] \cap \Omega = \emptyset$ as well.
  Therefore $\vd \cap \Omega = \emptyset$.

  To show the reverse direction, suppose that $\Omega$ is not a siphon.
  Then there is a reaction $\alpha=(\vr,\vp)$ such that $[\vp]$ contains an element $S \in \Omega$, but $[\vr] \cap \Omega = \emptyset$.
  Then from any state $\vc$ such that $[\vc] = \Lambda \setminus \Omega$ (i.e., all species not in $\Omega$ are present), $\alpha$ is applicable.
  Running $\alpha$ produces $S$, hence results in a state $\vd$ such that $\vc \segto \vd$ with $\Omega \cap [\vd] \neq \emptyset$, since $S \in \Omega$.
\end{proof}
}
\opt{normal,itcs}{\proofLemSegReachableForwardInvariantSiphon}

\newcommand{\lemMassActionReachable}{
  If $\vd$ is mass-action reachable from $\vc$, then $\vc \segto \vd$.
}

\begin{lemma}  \label{lem:mass-action-reachable}
  \lemMassActionReachable
\end{lemma}

\newcommand{\proofLemMassActionReachable}{
\begin{proof}
This proof is similar to the proof of Lemma~\ref{lem-reachable-segment-bound};
the main difference is that we need to define the ``reaction fluxes'' each reaction experiences on the mass-action trajectory from $\vc$ to $\vd$, and that we need to find an ordering on those reactions with positive flux that allows us to apply them one-by-one in order to show $\vc \segto^{m+1} \vd$.




\newcommand{\PROD}{\mathsf{PROD}}
\newcommand{\RXN}{\mathsf{RXN}}
%\repds{
%We first show that the set of species produced under mass-action is a subset of those producible under $\segto$.
%Let $C=(\Lambda,R)$ be the original CRN.
%Let $\Delta \subseteq \Lambda$.
%Define $\RXN(\Delta) = \setr{(\vr,\vp) \in R}{[\vr] \subseteq \Delta}$ to be the set of reactions that are applicable to any state with positive concentrations of species in $\Delta$.
%Define $\PROD(\Delta) = \{ S \in \Lambda \} \{ (\exists (\vr,\vp) \in \RXN(\Delta))\ S \in [\vp-\vr] \}$ to be the set of species \emph{produced} by reactions in $\RXN(\Delta)$.
%Let $\vc$ be a state.
%Define $\Lambda_0(\vc)=[\vc]$ and for all $i\in\N$, define $\Lambda_{i+1}(\vc) = \Lambda_i(\vc) \cup \PROD(\Lambda_i(\vc))$.
%Say that species $S\in\Lambda$ is \emph{eventually producible} from $\vc$ if there exists $i\in\N$ such that $S \in \Lambda_i(\vc)$.
%Define $R_i(\vc) = \RXN(\Lambda_i)$, and say that reaction $\alpha\in R$ is \emph{eventually applicable} from $\vc$ if there exists $i\in\N$ such that $\alpha \in R_i(\vc)$.
%Note that for large enough $i$, $\Lambda_{i}(\vc)=\Lambda_{i+1}(\vc)$ and $R_{i}(\vc)=R_{i+1}(\vc)$, ($i = |R|$ suffices).
%Denote the set of species eventually producible from $\vc$ as $\Lambda_\infty(\vc)$, and the set of reactions eventually applicable to $\vc$ as $R_\infty(\vc)$, i.e., $R_\infty(\vc) = \RXN(\Lambda_\infty(\vc))$.
%Note that for all $(\vr,\vp) \in R_\infty(\vc)$, $[\vr] \subseteq \Lambda_\infty(\vc)$ and $[\vp] \subseteq \Lambda_\infty(\vc)$.
%}{}


%\repds{
%Let $\Omega = \Lambda \setminus \Lambda_\infty(\vc)$.
%We claim that $\Omega$ is a siphon.
%This is established as follows.
%By the definition of $\Lambda_\infty(\vc)$, there is a state $\va$ such that $\vc \segto \va$ and $[\va]=\Lambda_\infty(\vc)$.
%Let $\vd$ be any state such that $[\va]=[\vd]$.
%We claim that no species in $\Omega$ is producible from $\vd$, i.e., by Lemma~\ref{lem-seg-reachable-forward-invariant-siphon}, $\Omega$ is a siphon.
%To see why, observe that since $[\va]=[\vd]$, there exists a constant $c \in \Rp$ such that $c\va \geq \vd$.
%If some element of $\Omega$ were producible from $c\va$, it would be producible by the same line segments, shrunk by factor $c$, from $\va$, so nothing in $\Omega$ is producible from $c\va$.
%However, producibility cannot be inhibited by adding extra amounts of species (since this can only make some reactions applicable but not make them inapplicable), so neither is anything in $\Omega$ producible from $\vd$, since $\vd \leq c \va$.
%%Clearly, $\Omega$ is a siphon.
%%If not, then there must be a reaction with all reactants in $\Lambda_\infty(\vc)$, but with a product not in $\Lambda_\infty(\vc)$, which contradicts the definition of $\Lambda_\infty(\vc)$.
%Since $\Omega$ is a siphon, by Lemma~\ref{lem-mass-action-forward-invariant-siphon}, no element of $\Omega$ is produced in any state $\vd$ mass-action reachable from $\vc$.
%}{}

First, suppose $\vd$ is reached in finite time $t_f$.
The trajectory followed by mass-action kinetics to get from $\vc$ to $\vd$ defines a differentiable curve $\rho:[0,t_f] \to \Rp^n$. % obeying Definition~\ref{defn-reachable-curve}.
Let $\rho' = \frac{d \rho}{dt}$ be the corresponding mass-action differential equations.
%Then for all $t$, $\rho'(t)$ is a nonnegative sum of reactions by property~\ref{defn-reachable-curve-prop2}.
%These reactions are eventually applicable by property~\ref{defn-reachable-curve-prop3}.
%\todo{I think $f_j$ and $\vu$ from above are related.}
Let the reactions $R$ be $\alpha_0, \alpha_1,\ldots.$
Let $f_j:[0,t_f] \to \Rp$ be the ``instantaneous flux'' through the $j$'th reaction at time $t$.
In other words, $\rho'(t) = \sum_{j} f_j(t) \vv_j$, where index $j$ ranges over all reactions, $\vv_j$ represents the $j$'th reaction vector ($\vp-\vr$ if $\alpha_j = (\vr,\vp)$, i.e., the $j$'th column of $\vM$).

By the fundamental theorem of calculus,
\opt{normal,submission}{
$$
    \vd - \vc
    = \rho(t_f) - \rho(0)
    =
    \int_0^{t_f} \rho'(t) dt
    =
    \int_0^{t_f} \sum_j f_j(t) \vv_j dt
    =
    \sum_j \vv_j \int_0^{t_f} f_j(t) dt,
$$
}
\opt{itcs,final}{
\begin{eqnarray*}
    \vd - \vc
    &=& \rho(t_f) - \rho(0)
    =
    \int_0^{t_f} \rho'(t) dt
    \\&=&
    \int_0^{t_f} \sum_j f_j(t) \vv_j dt
    =
    \sum_j \vv_j \int_0^{t_f} f_j(t) dt,
\end{eqnarray*}
}
Let $F_j = \int_0^{t_f} f_j(t) dt$ be the total flux through the $j$'th reaction.
Then $\vd = \vc + \sum_{j \in P} F_j \vv_j$.

If $\vd$ is not reached in finite time, then by the definition of mass-action reachability, $\vd = \lim_{t_f \to \infty} \rho(t_f)$.
Now, if we define $F_j = \int_0^{\infty} f_j(t) dt$ as above, the flux $F_j$ could be infinite (consider $X \lrevrxn Y$, which approaches the point with equal concentrations of $X$ and $Y$ but has infinite flux through each reaction in the limit).
Instead, we observe that for each species $S$ being produced by one reaction whose flux is going to infinity, there must be a corresponding reaction consuming $S$ whose flux is also going to infinity, for $\vd(S)$ to be finite.
Therefore we can find finite, positive values for each $F_j$ such that $\vd = \vc + \sum_{j \in P} F_j \vv_j$ as above.



Let $R_\rho = \setl{\alpha_j\in R}{F_j > 0}$ be the reactions that occurred with strictly positive flux along the curve $\rho$.
We claim that there is an ordering $\prec$ of reactions in $R_\rho$, such that for any reaction $\alpha=(\vr,\vp)$, $[\vr] \subseteq [\vc] \cup \bigcup_{\alpha'=(\vr',\vp') \prec \alpha} [\vp']$.

Let $\mathcal{S}_0, \dots, \mathcal{S}_l \subseteq \Lambda$ be a finite sequence of sets of species, and $\beta_1, \dots, \beta_l \in R_\rho$ be a finite sequence of reactions which are generated as follows.
Let $\mathcal{S}_0 = [\vc]$.
Given $\mathcal{S}_0, \dots, \mathcal{S}_{i-1}$ and $\beta_1, \dots, \beta_{i-1}$,
let $\beta_i$ be a new reaction in $R_\rho$ whose reactants are in $\mathcal{S}_{i-1}$,
and then form $\mathcal{S}_i$ by adding the products of $\beta_i$ to $\mathcal{S}_{i-1}$.
Let $\mathcal{S}$ be the final $\mathcal{S}_l$ such that we can no longer extend the sequence.
Call the reactions appearing in the list of $\beta$'s \emph{processed}.
If all of the reactions in $R_\rho$ are processed, then the order in which they are processed can define the ordering $\prec$.
We now claim that indeed all reactions in $R_\rho$ will be processed.


We proceed by contradiction:
we argue that the existence of an unprocessed reaction in $R_\rho$ contradicts Lemma~\ref{lem-mass-action-forward-invariant-siphon}.
Let $\overline{\mathcal{S}} = \Lambda \setminus \mathcal{S}$.
For all unprocessed reactions in $R_\rho$, at least one reactant is in $\overline{\mathcal{S}}$.
We also know that for all processed reactions in $R_\rho$, their products are not in $\overline{\mathcal{S}}$.
Thus $\overline{\mathcal{S}}$ is a siphon for the CRN consisting of reactions in $R_\rho$.
Let $S^*$ be a reactant of the unprocessed reaction in $R_\rho$, and let $F^*$ be its total flux.
We know that $F^* > 0$, and thus there must be a point in the mass-action trajectory where $S^*$ has positive concentration.
However, $\vc$ is zero on the siphon $\overline{\mathcal{S}}$, and $S^* \in \overline{\mathcal{S}}$.
%TODO: Different CRN!
This violates Lemma~\ref{lem-mass-action-forward-invariant-siphon}.


The sequence $\beta_1, \dots, \beta_l$ gives an ordering $\prec$ on reactions in $R_\rho$.
Using this ordering, the remainder of the proof is identical to the proof of Lemma~\ref{lem-reachable-segment-bound}.
\end{proof}
}

\opt{normal,itcs}{\proofLemMassActionReachable}



Lemma~\ref{lem:mass-action-reachable} shows that our definition of reachability is at least as general as mass-action kinetics.
In the other direction, ultimately we must appeal to intuition to justify that our definition does not reach too far.
Our intuition says that the following properties are required of any reasonable notion of reachability:
(1) concentrations must be nonnegative in all reachable states,
(2) a reaction cannot execute in any state in which some reactant is 0,\footnote{In particular, we want siphons to behave reasonably in that their absence is forward-invariant; i.e., that Lemmas~\ref{lem-mass-action-forward-invariant-siphon} and~\ref{lem-seg-reachable-forward-invariant-siphon} should apply to any reasonable notion of reachability.}
(3) the relation should be reflexive, transitive, and ``respect addition'' (if $\vx\to\vy$, then for all $\vc$, $\vx+\vc\to\vy+\vc$, since the presence of additional chemicals should not \emph{prevent} reactions from being possible).
Our definition was the most general one we could conceive that satisfied these properties.



Segment-reachability will serve as our main notion of reachability.
Hence, throughout the rest of the paper, we say $\vd$ is \emph{reachable} from $\vc$, written $\vc \to \vd$, if $\vc \segto \vd$.








\subsection{Stable computation}
\label{subsec-stable-crns}

In this section, we use our notion of reachability introduced above to formally define our notion of rate-independent computation.
Intuitively, devious rate laws might take the system along trajectories anywhere in the reachable space.
For the computation to be correct despite the rate laws, it must be able to reach a state with the final correct output from any reachable state.
Further, in this setting an output can reasonably be called final only if no rate law can falsify it.



First, to formally define what it means for such a CRN to compute a function, we must first single out some aspects of the CRN as semantically meaningful.
Formally, a \emph{chemical reaction computer (CRC)} is a tuple $\calC = (\Lambda,R,\Sigma,Y)$, where $(\Lambda,R)$ is a CRN, $\Sigma \subset \Lambda$, written as $\Sigma = \{X_1,\ldots,X_k\}$,\footnote{We assume a canonical ordering of $\Sigma=\{X_1,\ldots,X_k\}$ so that a vector $\vx\in\Rp^k$ (i.e., an input to $f$) can be viewed equivalently as a state $\vx\in\Rp^\Sigma$ of $\calC$ (i.e., an input to $\calC$).
Also, we have defined valid initial states to contain only the input species $\Sigma$; other species must have initial concentration 0.
Our results would change slightly if we relaxed this assumption; however, considering any species $S \not\in \Sigma$ as an ``auxiliary input'', the result would remain that what is computed is a (piecewise) linear function of those species present initially.
Since the initial value of non-input species would be constant across all valid initial states, rather than linear functions $f(\vx) = \sum_{i=1}^k a_i \vx(i)$, we would instead deal with \emph{affine} functions $f(\vx) = c + \sum_{i=1}^k a_i \vx(i)$, where the constant $c$ would depend only on the initial concentrations of non-input species.} is the \emph{set of input species}, and $Y \in \Lambda \setminus \Sigma$ is the \emph{output species}.
%Intuitively, $\calC$ computes a function $f:\Rp^k\to\Rp$ if, starting in a state with $\vx\in\Rp^k$ concentration of species in $\Sigma$, and concentration 0 of everything else, it is guaranteed (no matter the rate at which reactions proceed) to reach a state $\vo$ in which $\vo(Y) = f(\vx)$, and from that point on, no reactions can change the concentration of $Y$.


%\repds{
%Formally, let $f:\Rp^k \to \Rp$ be a function
%%\footnote{Our results extend easily to functions $f:\R^k \to \R^l$, i.e., whose output is a vector of $l$ real numbers.
%%This is because such a function is equivalently $l$ separate functions $f_i:\R^k\to\R$.}
%and let $\calC=(\Lambda,R,\Sigma,Y)$ be a CRC.
%We say that a state $\vo \in \Rp^\Lambda$ is \emph{output stable} if, for all $\vo'$ such that $\vo \to \vo'$, $\vo(Y) = \vo'(Y)$, i.e., once $\vo$ is reached, no reactions can change the concentration of $Y$.
%We say that $\calC$ \emph{stably computes} $f$ if, for all $\vx \in \Rp^k$, for all $\vc$ such that $\vx \to \vc$, there exists an output stable state $\vo$ such that $\vc \to \vo$ and $\vo(Y) = f(\vx)$.
%}{}



\begin{definition}
A state $\vo \in \Rp^\Lambda$ is \emph{output stable} if, for all $\vo'$ such that $\vo \to \vo'$, $\vo(Y) = \vo'(Y)$,  i.e., once $\vo$ is reached, no reactions can change the concentration of the output species $Y$.
\end{definition}


\begin{definition} \label{def:direct-computation}
Let $f:\Rp^k \to \Rp$ be a function\footnote{Our results extend easily to functions $f:\R^k \to \R^l$, i.e., whose output is a vector of $l$ real numbers.
This is because such a function is equivalently $l$ separate functions $f_i:\R^k\to\R$.}
and let $\calC$ be a CRC.
We say that $\calC$ \emph{stably computes} $f$ if, for all $\vx \in \Rp^k$, for all $\vc$ such that $\vx \to \vc$, there exists an output stable state $\vo$ such that $\vc \to \vo$ and $\vo(Y) = f(\vx)$.
\end{definition}








\subsection{Dual-rail representations}

In general, the output species of an upstream CRN may be used as the inputs to a downstream CRN if the upstream CRN only produces but never consumes the output species.
We say that such a CRN computes its output \emph{monotonically}.
This is impossible for general stable CRNs.
For example, any CRN computing the function $f(x_1,x_2) = x_1 - x_2$ must necessarily be able to consume its output species in order to account for some amount of species $X_2$ that has not yet reacted.
Therefore, some of our CRNs represent their output $Y$ in a ``dual-rail'' fashion as the difference of two species $Y^+$ and $Y^-$, both of which are only produced but never consumed by the CRN.
Since these outputs are given as input to a downstream subroutine CRN, the downstream CRN must also be designed to accept inputs in this same dual-rail representation.
Furthermore, representing values in this way allows us to take negative inputs and produce negative outputs, using only nonnegative concentrations, representing for example a negative output by a higher concentration of $Y^-$ than $Y^+$.

%\repds{
%Formally, let $X$ and $Y$ be any sets with a subtraction operation, and let $f:X \to Y$ be a function.
%A function $\hf:X \times X \to Y \times Y$ is a \emph{dual-rail representation} of $f$ if, for all $x^+,x^- \in X$, if $(y^+,y^-) = \hf(x^+,x^-)$, then $f(x^+ - x^-) = y^+ - y^-$.
%In other words, $\hf$ represents $f$ as the difference of its two outputs $y^+$ and $y^-$, and it works for any input pair $(x^+,x^-)$ whose difference is the input value to $f$.
%A function $\hf:X \to Y \times Y$ is an \emph{output dual-rail representation} of $f$ if, for all $x \in X$, if $(y^+,y^-) = \hf(x)$, then $f(x) = y^+ - y^-$.
%A function $\hf:X \times X \to Y$ is an \emph{input dual-rail representation} of $f$ if, for all $x^+,x^-$, $f(x^+ - x^-) = \hf(x^+,x^-)$.
%We can define a CRC to stably compute such a function in the same manner as in Section~\ref{subsec-negative-computable-implies-piecewise-linear}, but having input species $X_1^+,X_1^-,X_2^+,X_2^-,\ldots,X_k^+,X_k^-,\ldots,$ and two output species $Y^+$ and $Y^-$.}
Formally, let $f:\R^k \to \R$ be a function.
A function $\hf:\R^{2k} \to \R^2$ is a \emph{dual-rail representation} of $f$ if, for all $\vx^+,\vx^- \in \R^k$, if $(y^+,y^-) = \hf(\vx^+,\vx^-)$, then $f(\vx^+ - \vx^-) = y^+ - y^-$.
In other words, $\hf$ represents $f$ as the difference of its two outputs $y^+$ and $y^-$, and it works for any input pair $(\vx^+,\vx^-)$ whose difference is the input value to $f$.
We can define a CRC to stably compute such a function in the same manner as in Section~\ref{subsec-negative-computable-implies-piecewise-linear}, but having input species $X_1^+,X_1^-,X_2^+,X_2^-,\ldots,X_k^+,X_k^-,\ldots,$ and two output species $Y^+$ and $Y^-$.



\begin{definition}
We say that a CRC \emph{stably dual-computes} $f:\R^k \to \R$ if it stably computes a dual-rail representation $\hf:\R^k \times \R^k \to \R \times \R$ of $f$.
\end{definition}



%\repds{Note that if a CRN stably computes a dual-rail representation $\hf:\Rp^k \times \Rp^k \to \Rp \times \Rp$ of a function $f: \R^k \to \R$, it is straightforward to modify the CRN to compute an output dual-rail representation with the standard input convention, if the function's inputs are nonnegative.
%This is as simple as setting the initial concentration of $X_i^+$ to $\vx(i)$ and the initial concentration of $X_i^-$ to 0 (i.e., $X_i^+$ becomes the only input for the $i$'th coordinate).
%Similarly, if it never consumes its output species $Y^+$ and $Y^-$, an input dual-rail representation of $f$ is computable using the standard output convention: simply add the reaction $Y^+ + Y^- \to \emptyset.$
%%By using dual-rail inputs, we allow CRNs to compute functions with negative inputs and outputs, since such values can be specified by two nonnegative concentrations whose difference is negative.
%}
Note that if a CRC monotonically outputs $Y^+$ and $Y^-$ according to the dual-rail convention, and the output value is never negative, then it can be trivially modified to produce its output according to the direct computation convention (Def.~\ref{def:direct-computation}) by adding the reaction $Y^+ + Y^- \to \emptyset.$
%
%\repds{If a CRN computes a dual-rail representation $\hf:\R^k \times \R^k \to \R \times \R$ of some function $f:\R^k \to \R$, we say that the CRN \emph{stably dual-computes} $f$.}{}
%
%
Note that a single function has an infinite number of dual-rail representations.
We require only that a CRN exists to compute one of them to say that the function is stably dual-computable by a CRN.



==> biography.tex <==
\begin{IEEEbiographynophoto}{Cameron Chalk}
received the B.S. and M.S. degrees from the University of Texas Rio Grande Valley, Edinburg, TX, USA, in 2015 and 2017 respectively. He is currently pursing a Ph.D. degree from the University of Texas at Austin, TX, USA.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Niels Kornerup}
is an undergraduate working on B.S. degrees in both computer science and math at The University of Texas at Austin. He is planning on graduating in the Spring of 2020 to pursue a Ph.D. in theoretical computer science.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Wyatt Reeves}
is currently an undergraduate at the University of Texas at Austin, TX, USA, majoring in mathematics. 
\end{IEEEbiographynophoto}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{david-ieee}}]{David Soloveichik}
received the B.S. and M.S. degrees from Harvard University, Cambridge, MA, USA, in 2002 and the Ph.D. degree from the California Institute of Technology, Pasadena, CA, USA, in 2008. He is currently an Assistant Professor in the Department of Electrical and Computer Engineering at the University of Texas at Austin, TX, USA.
\end{IEEEbiography}

\vfill

==> correspondence.tex <==


\section{Stable computation under mass-action kinetics}
\label{sec:mass-action}

% \begin{definition}\label{feed-forward}
% A CRN $\calC = (\Lambda, R)$ is \emph{feedforward} if $\Lambda$ can be ordered as $\set{X_1, ..., X_n}$ so that for every reaction $r \in R$, if $r$ produces $X_i$, then it must consume some $X_j$, where $j < i$.
% \end{definition}

The definition of stable computation required that from any reachable state, the output stable state (with the correct answer) is reachable.
In this section we show that the CRC from Lemma~\ref{lem:full-construction} actually satisfies the following stronger condition: from any reachable state they \emph{converge} to the output stable state under \emph{mass-action kinetics}.
(Note that since mass-action reachability implies segment reachability, this is a stronger statement.)


We say a CRN is \emph{feedforward} if the species can be ordered so that every reaction that (net) produces $S_i$ also (net) consumes some $S_{i'}$ for $i' < i$. 
Formally:
\begin{definition}\label{feed-forward}
A CRN $\calC = (\Lambda, R)$ is \emph{feedforward} if $\Lambda=\set{S_1, ..., S_n}$ and its stoichiometry matrix satisfies $\vM(i,j) > 0 \Rightarrow \exists (i' < i) \vM(i',j) < 0$.
\end{definition}
The following lemma says that all mass-action equilibria (i.e., no concentration is changing) of feedforward CRNs are static (i.e., no reactions are firing, as opposed to multiple reactions firing with canceling effects).
\begin{lemma}\label{static-eq}
If a feedforward CRN $\calC$ is in a mass-action equilibrium $\vec{x}$ then no reaction is applicable at $\vec{x}$. 
\end{lemma}

\begin{proof}
Suppose there is at least one reaction which is applicable at $\vec{x}$. As a result, the set of all pairs $(i, j)$ where reaction $r_j$ is applicable and $\vM(i, j) > 0$ is non-empty. Take a pair $(i_0, j_0)$ where $i_0$ is chosen to be as small as possible. Since $\calC$ is feedforward and $\vM(i_0, j_0) > 0$, there is some $i' < i$ such that $\vM(i', j_0) < 0$. Furthermore, from our choice of $i$, we know that $\vM(i', j) \le 0$ for any applicable reaction $r_j$. As a result, $\frac{dS_{i'}}{dt} < 0$, so $\vec{x}$ is not a mass-action equilibrium.
\end{proof}


\begin{lemma}
Under mass-action kinetics, 
feedforward CRNs converge to some equilibrium point from any state.
\end{lemma}

1. Using the standard existence, uniqueness and regularity results for systems of first order ODEs found in \cite{leesmoothmanifolds}, because mass-action differential equations have rates of change that vary smoothly with the concentrations of all the species, for each point $x$ in the configuration space, there is a neighborhood $U$ of $x$ such that for all points $\vec{y} \in U$, there is a unique solution to the mass action equations starting at $\vec{y}$ for times in some range $(-\epsilon, \epsilon)$, and this solution varies smoothly both with respect to time and with respect to $\vec{y}$.

2. Because the CRN is feed-forward, it is mass non-increasing, so for any initial species concentration in $\mathbb{R}^n_{\ge 0}$, the solution to the mass action equations is contained inside of a compact subset $K$ of $\mathbb{R}^n$.

3. Since $K$ is compact, it is covered by finitely many of the neighborhoods from 1, so there is a minimum $\epsilon'$ such that the ODE has a solution around each point in $K$ for all times in $(-\epsilon', \epsilon')$. This implies the existence of a globally defined solution for any point in $K$.

4. By the smoothness condition from 1, starting at an initial point $\vec{z}$, the solution to the mass action ODE is a smooth function $\gamma: \mathbb{R} \to K$. In particular, the first derivative of $\gamma$ exists, and we know that $\gamma'(t) = \sum_{j} f_j^{\vec{z}}(t)\vec{v}_j$, where $f_j^{\vec{z}}$ is the flux through reaction $j$ at time $t$ and $\vec{v}_j$ is the $j$-th column of the stoichiometry matrix. 

5. Because the CRN that we have constructed is feed-forward, we know that $\int_0^\infty f_j^{\vec{z}}(t) dt < \infty$, so we know that 

\[\int_0^\infty |\gamma'(t)| dt = \int_0^\infty \left|\sum_{j} f_j^{\vec{z}}(t)\vec{v}_j\right| dt \le \int_0^\infty \sum_{j} f_j^{\vec{z}}(t)|\vec{v}_j| dt\]
\[= \sum_{j}|\vec{v}_j| \int_0^\infty  f_j^{\vec{z}}(t) dt < \infty\]

In other words, $\gamma$ has finite length.

6. Suppose that there is some $\epsilon > 0$ such that for all $M \in \mathbb{R}_{\ge 0}$, there exists some $t > s > M$ such that $d(\gamma(t), \gamma(s)) \ge \epsilon$. Then take $M_1 = 0$, and label the points we get by this assumption $t_1, s_1$. Then for any $n > 1$, take $M_n = t_{n-1}$ and label the next pair of points $t_n, s_n$. Then 

\[\int_0^\infty |\gamma'(t)| dt \ge \sum_{i = 1}^\infty \int_{s_i}^{t_i}|\gamma'(t)| dt \ge \sum_{i = 1}^\infty d(\gamma(t_i), \gamma(s_i)) \ge \sum_{i = 1}^\infty \epsilon = \infty \]

This contradicts 5, so for all $\epsilon > 0$, there is some $M \in \mathbb{R}_{\ge 0}$ such that for all $t, s > M$, we know $d(\gamma(t), \gamma(s)) < \epsilon$.

7. From 6, we know that if $\vec{x}_k = \gamma(k)$, then $\set{\vec{x}_k}_{k = 1}^\infty$ is a Cauchy sequence in $\mathbb{R}^n$, so it must converge to some point $\vec{x}_0$. From 6 and the convergence of $\vec{x}_n$ to $\vec{x}_0$, we conclude that $\gamma(t) \to \vec{x}_0$ as $t \to \infty$.

8. Because the flow is smooth from 1, it is in particular continuous, so $\vec{x}_0$ must be an equilibrium point. This is because for any $t$ and any $\epsilon > 0$, we can choose a suitable point $\vec{y}$ in $\gamma$ such that $d(\gamma_{\vec{x_0}}(t), \gamma_{\vec{y}}(t)) < \epsilon/2$ and $d(\vec{x_0}, \gamma_{\vec{y}}(t)) < \epsilon/2$, so that $d(\vec{x_0}, \gamma_{\vec{x_0}}(t)) < \epsilon$.

9. Since the CRN we constructed is feed-forward, $\vec{x}_0$ must actually be a static equilibrium point, so it is output stable. Since $\vec{x}_0$ is mass-action reachable from $\vec{z}$, it is segment reachable, and because the CRN output-stably computes the desired function, $\vec{x}_0$ must have the correct amount of the output species present.

==> direct_vs_dualrail.tex <==


\subsection{Direct vs. Dual-Rail}\label{sec:dual-rail}
\todoi{CC: Already moved some dual-rail discussion to intro; maybe we can remove this whole section (5.1) and leave the discussion in the intro. (For space)}
% We note that our results apply to the ``direct'' input and output representation, where the concentration of a species carrying the signal is the signal value. 
% An alternative representation called dual-rail, previously used in the literature, encodes a value by the difference of the concentration of two species~\cite{rate-indep}.
% Requiring composability for the dual-rail representation does not restrict computational power of rate-independent CRNs.
% Intuitively, this is because the logical value of an output can be decreased by increasing concentration of the subtracted species.
%\todoi{CC: What can we say here about general encoding schemes? E.g., dual-rail removes superadditivity constraint, but what other conventions do? I don't think this is as obvious as it was in the meeting}

==> discontinuous_functions.tex <==
\section{Fuzzy Stable Computation: Allowing Incorrectness on Few Inputs}\label{sec:discontinuity}
It has been shown that functions computable by rate-independent CRNs must be continuous.
However, if one allows CRCs to err on a small set of inputs, and the function is discontinuous only on these sets, the function may be computable. 
For example, consider the non-composable CRN:
\begin{align}
    X_1 + X_2 &\rxn Y \\
    X_1 + Y &\rxn X_1 + B\\
    X_2 + B &\rxn X_2 + Y
\end{align}
which computes the discontinuous function
\begin{equation}\label{eq:example}
f(x_1, x_2) = \begin{cases} 
      0 & x_1 \geq x_2 \nonumber \\
      x_1 & x_1 < x_2
   \end{cases}
\end{equation}
\noindent
everywhere except where $x_1 = x_2$. 
If $x_1 > x_2$, from any reachable state, fire the first reaction until completion, resulting in zero $X_2$ and some positive amount of $X_1$.
Then fire reaction two until all $Y$ is converted into $B$. Then no reaction can fire, so the state is output stable with zero $Y$.
If $x_1 < x_2$, fire the first reaction until completion.
Now we can fire reaction three until all $B$ is converted into $Y$; the amount of $Y$ produced in total is $x_1$.
However, if $x_1 = x_2$, an output stable state with concentration of $Y$ between $0$ and $x_1 = x_2$ can be reached. Thus slightly loosening the definition of stable computation---allowing incorrect output on a domain of measure zero---allows a wider class of computable functions.

This example, however, is not composable. In the composable case, we argue that allowing error on small subsets does not give more power.
First, we formally state a version of \emph{fuzzy} stable computation which allows the CRC to err on a subset of inputs:
\begin{definition}
Let $f:\Rp^n \to \Rp$ be a function, let $\calC$ be a CRC, and let $M \subset \Rp^n$.
We say that $\calC$ \emph{$M$-fuzzy stably computes} $f$ if, for all $\vx \in \Rp^n \setminus M$, and all $\vc$ such that $\vx \to \vc$, there exists an output stable state $\vo$ such that $\vc \to \vo$ and $\vo(Y) = f(\vx)$.
\end{definition}
\todoi{CC: Definition should be for general error subsets.
For lemma, the error subset should be finite union of linear relationships between inputs }
\begin{lemma}
Let $M$ be the union of a finite number of vector spaces in $\mathbb{R}^n$. If an output-oblivious CRC $\calC$ $M$-fuzzy stably computes $f$, then $f$ must be superadditive piecewise rational linear over $\mathbb{R}_{\geq 0}^n \setminus M$.
\end{lemma}
\todoi{prove this - It should just follow from the cone argument. Superadditivity might need to be redefined as well.}

==> table_previous_work.tex <==
\begin{center}
\begin{tabular}{ | c | c | c | c | }
\hline
\textbf{Representation} & \textbf{Composable} & \textbf{Functions}  &
 \textbf{Reference}\\\hline
\multicolumn{4}{c}{\textbf{Discrete Model}}\\ \hline
 \\\hline
 Direct & No & Semilinear &  \\ \hline 
 Direct & Yes & ? & N/A \\ \hline
 Dual-Rail & Yes & Semilinear & \\ \hline
 \\\hline
 \multicolumn{4}{c}{\textbf{Continuous Model}}\\ \hline
 Direct & No & Positive-Continuous Piecewise Rational Linear &  \\ \hline
 Direct & Yes & S$^+$ $+$-Cts. Piecewise Rational Linear &  \\ \hline
 Dual-Rail & Yes & Continuous Piecewise Rational Linear &  \\
 \hline
\end{tabular}
\end{center}
